Measurement of the differential cross-section of highly boosted top quarks as a function of their transverse momentum in $\sqrt{s}$ = 8 TeV proton-proton collisions using the ATLAS detector

The differential cross-section for pair production of top quarks with high transverse momentum is measured in 20.3 fb$^{-1}$ of proton-proton collisions at a center-of-mass energy of 8 TeV. The measurement is performed for $t\bar{t}$ events in the lepton+jets channel. The cross-section is reported as a function of the hadronically decaying top quark transverse momentum for values above 300 GeV. The hadronically decaying top quark is reconstructed as an anti-$k_t$ jet with radius parameter $R=1.0$ and identified with jet substructure techniques. The observed yield is corrected for detector effects to obtain a cross-section at particle level in a fiducial region close to the event selection. A parton-level cross-section extrapolated to the full phase space is also reported for top quarks with transverse momentum above 300 GeV. The predictions of a majority of next-to-leading-order and leading-order matrix-element Monte Carlo generators are found to agree with the measured cross-sections.

==> defs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%&&&&&&&&&&
% SPECIAL NEW COMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands from RH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PLEASE USE CHEIFLY THESE DEFINITIONS WHEN TYPING TOP KINEMATIC VARIABLES AND CROSS SECTIONS! %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ttb}{\ensuremath{{\ttbar}}}
\newcommand{\dm}{\ensuremath{{ d}m}}
\newcommand{\dmttbar}{\ensuremath{{ d}m_{\ttbar}}}
\newcommand{\yttbar}{\ensuremath{y_{\ttbar}}}
\newcommand{\absyttbar}{\ensuremath{\left|y_{\ttbar}\right|}\xspace}
\newcommand{\yt}{\ensuremath{y_{t}}}
\newcommand{\absyt}{\ensuremath{\left|y_{t}\right|}\xspace}
\newcommand{\dyttbar}{\ensuremath{{ d}y_{\ttbar}}}
\newcommand{\dabsyttbar}{\ensuremath{{ d}\absyttbar}\xspace}
\newcommand{\mttbar}{\ensuremath{m_{\ttbar}}}
\newcommand{\mt}{\ensuremath{m_{\mathrm{t}}}}
\newcommand{\dpt}{\ensuremath{{ d}p_{\rm T}}}
\newcommand{\dptttbar}{\ensuremath{{ d}\pt^{\ttbar}}}
\newcommand{\dsigma}{\ensuremath{{ d}\sigma}}
\newcommand{\ptt}{\ensuremath{\pt^t}}
\newcommand{\dptt}{\ensuremath{{ d}\pt^t}}
\newcommand{\dX}{\ensuremath{{ d}X}}
\newcommand{\ptttbar}{\ensuremath{\pt^{\ttbar}}}
\newcommand{\Etmiss}{\ensuremath{\ET^{\rm miss}}}
\newcommand{\Ht}{\ensuremath{H_{\rm T}}}
\newcommand{\Meff}{\ensuremath{m_{\rm eff}}}

% see http://tex.stackexchange.com/questions/31091/space-after-latex-commands
\newcommand{\ejets}{{$e+$jets}\xspace}
\newcommand{\mujets}{{$\mu+$jets}\xspace}
\newcommand{\ljets}{{$\ell+$jets}\xspace}

\newcommand{\mjjj}{\mbox{$m_{\rm jjj}$}}
\newcommand{\AKT}{anti-$k_{t}$}
\newcommand{\Zg}{\Zboson/\gamma^*}
\def\lum{{\cal L}}
\newcommand{\muplus} {\ensuremath{\mu+\mathrm{jets}}\xspace}
\newcommand{\eplus} {\ensuremath{e+\mathrm{jets}}\xspace}
\newcommand{\lplus} {\ensuremath{\ell+\mathrm{jets}}\xspace}
\newcommand{\nl} {N^{\mathrm{loose}}}
\newcommand{\nlr} {N^{\mathrm{loose}}_{\mathrm{real}}}
\newcommand{\nlf} {N^{\mathrm{loose}}_{\mathrm{fake}}}
\newcommand{\nt} {N^{\mathrm{tight}}}
\newcommand{\ntr} {N^{\mathrm{tight}}_{\mathrm{real}}}
\newcommand{\ntf} {N^{\mathrm{tight}}_{\mathrm{fake}}}
\newcommand{\epsr} {\ensuremath{\epsilon_{\mathrm{real}}}}
\newcommand{\epsf} {\ensuremath{\epsilon_{\mathrm{fake}}}}
\newcommand{\dr} {\ensuremath{\Delta R({\rm lepton},{\rm jet})}}
\newcommand{\pmasym}[2]{^{+#1}_{-#2}}
\newcommand{\sigmattbar}{\ensuremath{\sigma_{\ttbar}}}

\newcommand{\sigtt}{\ensuremath{\sigma_{\ttbar}}\xspace}
\newcommand{\wjets}{\ensuremath{W\!+\!\mathrm{jets}}\xspace}
\newcommand{\zjets}{\ensuremath{Z\!+\!\mathrm{jets}}\xspace}
\newcommand{\ej}{\ensuremath{e+\mathrm{jets}}\xspace}
\newcommand{\mj}{\ensuremath{\mu+\mathrm{jets}}\xspace}
\newcommand{\njets}{\ensuremath{N_{\mathrm{jets}}}\xspace}
\newcommand{\expA}{\ensuremath{\exp[-8\times A]}\xspace}
\newcommand{\Http}{\ensuremath{H_{\mathrm{T,3p}}}\xspace}
\newcommand{\expH}{\ensuremath{\exp[-4\times\Http]}\xspace}
\newcommand{\etal}{\ensuremath{\eta^{\ell}}\xspace}
\newcommand{\absetal}{\ensuremath{|\etal|}\xspace}
\newcommand{\wSV}{\ensuremath{w_{\mathrm{SVO}}}\xspace}
\newcommand{\wSVmean}{\ensuremath{\overline{w}_{\mathrm{SVO}}}\xspace}
\newcommand{\jprob}{\texttt{JetProb}\xspace}
\newcommand{\wJP}{\ensuremath{w_{\mathrm{JP}}}\xspace}
\newcommand{\wJPmean}{\ensuremath{\overline{w}_{\mathrm{JP}}}\xspace}

\newcommand{\UN}[2]{\mbox{$ #1 \; \rm{#2} $}}
\newcommand{\EQ}[3]{
\begin{eqnarray}
\label{#1}
#2\;\;#3
\end{eqnarray}
}

%
\newcommand{\mtw}{\ensuremath{m_{\mathrm{T}}^W}}

% new comands for this analysis
%\newcommand{\PtTop}{\ensuremath{p_{\mathrm{T,t}}}}
\newcommand{\Gt     }{\ensuremath{\Gamma_{\mathrm{top}}}}
\newcommand{\mtr    }{\ensuremath{\mt^{\mathrm{reco}}}}
% b-tag newcommands
%\newcommand{\btag   }{\ensuremath{b\mbox{-tagging}}\xspace}
%\newcommand{\btagged}{\ensuremath{b\mbox{-tagged}}\xspace}
%\newcommand{\bjet   }{\ensuremath{b\mbox{-jet}}\xspace}
%\newcommand{\bjets  }{\ensuremath{b\mbox{-jets}}\xspace}
%\newcommand{\bquark }{\ensuremath{b\mbox{-quark}}\xspace}
%\newcommand{\bquarks}{\ensuremath{b\mbox{-quarks}}\xspace}
%\newcommand{\kt     }{\ensuremath{k_\mathrm{t}}\xspace}

\newcommand{\btag   }{\ensuremath{b\mbox{-tagging}}\xspace}
\newcommand{\btagged}{\ensuremath{b\mbox{-tagged}}\xspace}
\newcommand{\bjet   }{\ensuremath{b\mbox{-jet}}\xspace}
\newcommand{\bjets  }{\ensuremath{b\mbox{-jets}}\xspace}
\newcommand{\bquark }{\ensuremath{b\mbox{-quark}}\xspace}
\newcommand{\bquarks}{\ensuremath{b\mbox{-quarks}}\xspace}
\newcommand{\kt     }{\ensuremath{k_\mathrm{t}}\xspace}
%

% from the top epjc paper

%\newcommand{\lumitot}{\mbox{2.9\,pb$^{-1}$}}

%\newcommand{\ncandlj}{37}
%\newcommand{\ncandll}{9}

%\newcommand{\nbglj}{\ensuremath{12.2 \pm 3.9}}
%\newcommand{\nbgll}{\ensuremath{2.5 \pm 0.6}}

%\newcommand{\sigcomb}{4.8}

%\newcommand{\xsecctot}{145}
%\newcommand{\xseccstat}{\pm 31}
%\newcommand{\xseccsyst}{~{}^{+42}_{-27}}

%\newcommand{\singlefigure}[4]{
%\begin{figure}[htbp]
%\centering
%\includegraphics[width=#2]{#1}
%\caption{\label{#3}#4}
%\end{figure}
%}

%\newcommand{\doublefigure}[6]{
%\begin{figure}[htbp]
%\includegraphics[width=#2]{#1}
%\includegraphics[width=#4]{#3}
%\caption{\label{#5}#6}
%\end{figure}
%}

\hyphenation{so-le-noid}
\hyphenation{re-con-struc-ted}

% new commands from fitting
%\newcommand{\Gt}{\ensuremath{\Gamma_{\mathrm{top}}}\xspace}


% quantities used in text
%  total integrated luminosity
\newcommand{\lumitot}{\mbox{4.6\,fb$^{-1}$}}
\newcommand{\lumitotAndError}{\mbox{4.6$\pm$0.085\,fb$^{-1}$}}
\newcommand{\invfb}{\mbox{fb$^{-1}$}}
% numbers of candidates in semileptonic and dileptonic
\newcommand{\ncandlj}{NN}
\newcommand{\ncandll}{MM}

% background estimates with total errors
\newcommand{\nbglj}{\ensuremath{XX\pm YY}}
\newcommand{\nbgll}{\ensuremath{XX\pm YY}}

% combined significance
\newcommand{\sigcomb}{5.1}

% final combined cross-section and errors
% note include \pm in errors in case we go asymmetric
\newcommand{\xsecctot}{XXX}
\newcommand{\xseccstat}{\pm YYY}
\newcommand{\xseccsyst}{\pm ZZZ}
\newcommand{\xsecclumi}{\pm XYZ}


% \newcommand{\}{{\sc }\xspace}

%%% please consider using these definitions throughout the text consistently;-) %%%
\newcommand{\RooUnfold}{{\sc RooUnfold}\xspace}
\newcommand{\Alpgen}{{\sc Alpgen}\xspace}
\newcommand{\Powheg}{{\sc Powheg}\xspace}
\newcommand{\PowHeg}{{\sc Powheg}\xspace}
\newcommand{\PowhegBox}{{\sc POWHEG-BOX}\xspace}
%\newcommand{\MCFM}{{\sc MCFM}\xspace}
\newcommand{\Jimmy}{{\sc Jimmy}\xspace}
\newcommand{\Pythia}{{\sc Pythia}\xspace}
\newcommand{\PythiaEight}{{\sc Pythia8}\xspace}
\newcommand{\Herwig}{{\sc Herwig}\xspace}
\newcommand{\Guru}{{\sc GURU}\xspace}
%\newcommand{\MCatNLO}{{\sc MC{@}NLO}\xspace}
\newcommand{\McAtNlo}{{\sc MC{@}NLO}\xspace}
\newcommand{\AtlFast}{{\sc AltFastII}\xspace}
\newcommand{\AcerMC}{{\sc AcerMC}\xspace}

\newcommand{\singlefigure}[5]{
\begin{figure}[tbp]
\centering
\includegraphics[width=#2]{#1}

\caption{\label{#3}#4}
\end{figure}
}

\newcommand{\doublefigure}[6]{
\begin{figure}[tbp]
\includegraphics[width=#2]{#1}
\includegraphics[width=#4]{#3}
\caption{\label{#5}#6}
\end{figure}
}

